ECDSA.Fail: Open Autoresearch for Optimizing Elliptic-Curve Point Addition in Shor's Algorithm

We propose Open Autoresearch, a paradigm in which humans and AI agents publish evaluator-verified improvements to a public leaderboard. We instantiate it in ECDSA.Fail, optimizing reversible secp256k1 point-addition circuits, a bottleneck in Shor's algorithm for elliptic-curve cryptography. The benchmark minimizes the spacetime-inspired score $S=Q\times T$, where $Q$ is peak logical qubit width and $T$ is average executed Toffoli count. Participants reduced $S$ by 86.1%. At the data cutoff (26 July 2026), the best-scoring circuit uses 1,151 qubits and 1,299,453 average executed Toffoli gates, giving $Q\times T\approx1.496$ billion. This is more than 50% below Google's published point-addition score thresholds (arXiv:2603.28846), under different accounting conventions. Because the benchmark supplies one addend classically, we construct a coherent windowed-addition-compatible variant implementing the single-call interface required by windowed Shor. It uses 1,162 qubits and 1,684,161 average executed Toffoli gates. On 100,000 random inputs, its empirical success probability is $\hat{p}=0.99809$, giving $Q\times T/\hat{p}\approx1.961$ billion under an independently rerunnable per-call sensitivity model, not a full-Shor success estimate. Its qubit and Toffoli counts lie below Google's published thresholds and Schrottenloher's reported operating points (arXiv:2606.02235), although differing interfaces, accounting conventions, and validation scope preclude formal dominance. After the cutoff, the score was further reduced to 1.259 billion, while a separate low-width circuit reached 813 qubits. The public record shows AI agents complementing human judgment, providing evidence for open autoresearch on efficiently evaluable, machine-checkable objectives.

==> figs/circuit-resource-profile.tex <==
% Figure fragment: circuit resource profile.
% Input from within a figure environment in the main document.
% Requires tikz (with the backgrounds library), pgfplots, and pgfplotstable
% (loaded in tex_files/ZZ_header.tex).
% Reads the deposited phase CSVs from figs/circuit_profile_phases/. The current
% paper artifact does not yet include the raw profile trace or phase-splitting
% generator; evidence/verify_section5_claims.py reconciles the deposited tables
% with their longitudinal endpoint.
\definecolor{scoreblue}{HTML}{0072B2}
\definecolor{adjustedorange}{HTML}{D55E00}
\definecolor{phasegray}{HTML}{D8E0E6}
\definecolor{ink}{HTML}{24313A}

\IfFileExists{figs/circuit_profile_phases/coord_sub.csv}
  {\def\ProfilePhaseDir{figs/circuit_profile_phases}}
  {\def\ProfilePhaseDir{circuit_profile_phases}}

% Validate expected bin counts while loading the six phase tables.
\newcommand{\LoadAndCheckPhase}[3]{%
  \pgfplotstableread[col sep=comma]{\ProfilePhaseDir/#1.csv}#2%
  \pgfplotstablegetrowsof{#2}%
  \pgfmathtruncatemacro{\ProfilePhaseRows}{\pgfplotsretval}%
  \ifnum\ProfilePhaseRows=#3\else
    \PackageError{circuit_resource_profile}
      {Phase #1: expected #3\space rows, found \ProfilePhaseRows}
      {Regenerate figs/circuit_profile_phases with figs/split_circuit_profile.py.}
  \fi
}

\LoadAndCheckPhase{coord_sub}{\profileCoordSub}{96}
\LoadAndCheckPhase{inverse}{\profileInverse}{288}
\LoadAndCheckPhase{add3x}{\profileAddThreeX}{96}
\LoadAndCheckPhase{square}{\profileSquare}{288}
\LoadAndCheckPhase{multiply}{\profileMultiply}{288}
\LoadAndCheckPhase{coord_final}{\profileCoordFinal}{96}

\newcommand{\NarrowPhaseWidth}{0.88}
\newcommand{\InversePhaseWidth}{4.984501680}
\newcommand{\AddThreeXPhaseWidth}{0.045008725}
\newcommand{\SquarePhaseWidth}{0.755102370}
\newcommand{\MultiplyPhaseWidth}{4.775387224}
\newcommand{\PlotLeft}{1.05}
\newcommand{\ActiveBottom}{8.52}
\newcommand{\ToffoliBottom}{6.18}

\pgfplotsset{
  profile active left/.style={
    axis y line*=left,
    ytick={512,768,1024,1152},
    ylabel={Qubits},
    ylabel style={text=scoreblue,font=\small},
    yticklabel style={text=scoreblue,font=\scriptsize},
    y axis line style={scoreblue,line width=0.7pt},
    y tick style={scoreblue},
  },
  profile active hidden/.style={
    axis y line=none,
    ytick={512,768,1024,1152},
    yticklabels=\empty,
    y tick style={draw=none},
  },
  profile toffoli right/.style={
    axis y line*=right,
    ytick={0,1.041393,2.004321,3.000434,4.000043},
    yticklabels={$0$,$10$,$10^2$,$10^3$,$10^4$},
    ylabel={Toffoli},
    ylabel style={text=adjustedorange,font=\small},
    yticklabel style={text=adjustedorange,font=\scriptsize},
    y axis line style={adjustedorange,line width=0.7pt},
    y tick style={adjustedorange},
  },
  profile toffoli hidden/.style={
    axis y line=none,
    ytick={0,1.041393,2.004321,3.000434,4.000043},
    yticklabels=\empty,
    y tick style={draw=none},
  },
}

\newcommand{\PhasePlot}[7]{%
  % #1 = phase table macro, #2 = x-shift (cm), #3 = width (cm),
  % #4 = xmin, #5 = xmax, #6 = active y-axis style, #7 = toffoli y-axis style
  \pgfmathsetmacro{\PhaseShift}{#2}%

  % Upper band: active qubits. Only the first facet carries the left y-axis.
  \begin{axis}[
    at={({\PhaseShift cm},{\ActiveBottom cm})},
    anchor=south west,
    width=#3 cm,
    height=3.26cm,
    scale only axis,
    xmin=#4,
    xmax=#5,
    ymin=480,
    ymax=1180,
    axis x line=none,
    #6,
    xmajorgrids=false,
    ymajorgrids=false,
    clip=true,
    clip mode=individual,
    unbounded coords=jump,
  ]
    \addplot[
      scoreblue,
      line width=0.88pt,
      line join=round,
      no marks,
    ] table[
      x=local_index,
      y=active_qubit_count_per_index,
    ] {#1};
  \end{axis}

  % Lower band: mean executed Toffolis per complete run in each phase-local
  % time bin. Only the last facet carries the
  % independent right y-axis, so the two metric curves cannot intersect.
  \begin{axis}[
    at={({\PhaseShift cm},{\ToffoliBottom cm})},
    anchor=south west,
    width=#3 cm,
    height=1.70cm,
    scale only axis,
    xmin=#4,
    xmax=#5,
    ymin=0,
    ymax=4.02,
    axis x line*=bottom,
    xtick=\empty,
    x axis line style={ink!75,line width=0.45pt},
    #7,
    ymajorgrids=false,
    clip=true,
    clip mode=individual,
    unbounded coords=jump,
  ]
    \addplot[
      adjustedorange,
      line width=0.78pt,
      line join=round,
      no marks,
    ] table[
      x=local_index,
      y=log10_toffoli,
    ] {#1};
  \end{axis}
}

\tikzset{
  wire/.style={draw=ink,line width=0.62pt},
  gate/.style={
    draw=ink,
    fill=white,
    rounded corners=1.2pt,
    line width=0.62pt,
    minimum width=0.88cm,
    minimum height=0.62cm,
    inner sep=2pt,
    font=\small
  },
  twowiregate/.style={
    gate,
    minimum width=1.12cm,
    minimum height=2.06cm,
    align=center
  },
  phaseconnector/.style={
    draw=gray!55,
    dash pattern=on 2pt off 2pt,
    line width=0.45pt,
    line cap=round
  }
}

\newcommand{\PhaseGuidePair}[3]{%
  \draw[phaseconnector]
    (#1,5.94)
    .. controls (#1,5.60)
       and ($(#3.north west)+(0,0.26)$) ..
    (#3.north west);
  \draw[phaseconnector]
    (#2,5.94)
    .. controls (#2,5.60)
       and ($(#3.north east)+(0,0.26)$) ..
    (#3.north east);
}

\begin{tikzpicture}[x=1cm,y=1cm]
  % Exact final-operation spans of the four central phases. Their widths are
  % proportional to these spans, giving all four one common index scale.
  \pgfmathsetmacro{\xA}{\PlotLeft}
  \pgfmathsetmacro{\xB}{\xA+\NarrowPhaseWidth}
  \pgfmathsetmacro{\xC}{\xB+\InversePhaseWidth}
  \pgfmathsetmacro{\xD}{\xC+\AddThreeXPhaseWidth}
  \pgfmathsetmacro{\xE}{\xD+\SquarePhaseWidth}
  \pgfmathsetmacro{\xF}{\xE+\MultiplyPhaseWidth}
  \pgfmathsetmacro{\PlotRight}{\xF+\NarrowPhaseWidth}

  \node[font=\large,text=ink] at
    ({(\PlotLeft+\PlotRight)/2},12.72)
    {Circuit resource profile};

  % The edge coordinate phases remain independently compressed; the central
  % four phases share the common operation-index scale defined above.
  \begin{scope}[on background layer]
    \fill[ink!1.8]         (\xA,5.96) rectangle (\xB,12.02);
    \fill[scoreblue!2.5]   (\xB,5.96) rectangle (\xC,12.02);
    \fill[ink!1.8]         (\xC,5.96) rectangle (\xD,12.02);
    \fill[scoreblue!2.5]   (\xD,5.96) rectangle (\xE,12.02);
    \fill[ink!1.8]         (\xE,5.96) rectangle (\xF,12.02);
    \fill[scoreblue!2.5]   (\xF,5.96) rectangle (\PlotRight,12.02);

    % Single full-width horizontal guides. These are drawn independently of
    % the six phase facets so they cannot stop at a phase boundary.
    \foreach \tickvalue in {512,768,1024,1152} {
      \pgfmathsetmacro{\guidey}
        {\ActiveBottom+3.26*(\tickvalue-480)/(1180-480)}
      \draw[ink!14,line width=0.28pt]
        (\PlotLeft,\guidey) -- (\PlotRight,\guidey);
    }
    \foreach \tickvalue in {1.041393,2.004321,3.000434,4.000043} {
      \pgfmathsetmacro{\guidey}
        {\ToffoliBottom+1.70*\tickvalue/4.02}
      \draw[ink!14,line width=0.28pt]
        (\PlotLeft,\guidey) -- (\PlotRight,\guidey);
    }
  \end{scope}

  \PhasePlot{\profileCoordSub}{\xA}{\NarrowPhaseWidth}{0}{95}
    {profile active left}{profile toffoli hidden}
  \PhasePlot{\profileInverse}{\xB}{\InversePhaseWidth}{0}{287}
    {profile active hidden}{profile toffoli hidden}
  \PhasePlot{\profileAddThreeX}{\xC}{\AddThreeXPhaseWidth}{0}{95}
    {profile active hidden}{profile toffoli hidden}
  \PhasePlot{\profileSquare}{\xD}{\SquarePhaseWidth}{0}{287}
    {profile active hidden}{profile toffoli hidden}
  \PhasePlot{\profileMultiply}{\xE}{\MultiplyPhaseWidth}{0}{287}
    {profile active hidden}{profile toffoli hidden}
  \PhasePlot{\profileCoordFinal}{\xF}{\NarrowPhaseWidth}{0}{95}
    {profile active hidden}{profile toffoli right}

  % Shared plot frame, split between metrics to guarantee non-intersection.
  \draw[ink!55,line width=0.45pt]
    (\PlotLeft,5.96) rectangle (\PlotRight,12.02);
  \draw[ink!70,line width=0.35pt]
    (\PlotLeft,8.20) -- (\PlotRight,8.20);
  \foreach \xb in {\xB,\xC,\xD,\xE,\xF} {
    \draw[ink!32,line width=0.38pt] (\xb,5.96) -- (\xb,12.02);
  }

  % Regular ticks make the shared scale of the central four phases explicit.
  \foreach \offset/\lab in {
    2.156584961/$2\mathrm{M}$,
    4.327511059/$4\mathrm{M}$,
    6.498437157/$6\mathrm{M}$,
    8.669363256/$8\mathrm{M}$
  } {
    \pgfmathsetmacro{\xtick}{\xB+\offset}
    \draw[ink!70,line width=0.38pt] (\xtick,5.96) -- (\xtick,5.86);
    \node[anchor=north,font=\tiny,text=ink!82] at (\xtick,5.84) {\lab};
  }
  \node[anchor=north,font=\tiny,text=ink!82] at
    ({(\xA+\xB)/2},5.84) {$0\!-\!13.2\mathrm{k}$};
  \node[anchor=north,font=\tiny,text=ink!82] at
    ({(\xF+\PlotRight)/2},5.84) {$9.74\!-\!9.76\mathrm{M}$};
  \pgfmathsetmacro{\pA}{(\xA+\xB)/2}
  \pgfmathsetmacro{\pB}{(\xB+\xC)/2}
  \pgfmathsetmacro{\pC}{(\xC+\xD)/2}
  \pgfmathsetmacro{\pD}{(\xD+\xE)/2}
  \pgfmathsetmacro{\pE}{(\xE+\xF)/2}
  \pgfmathsetmacro{\pF}{(\xF+\PlotRight)/2}
  % The add3x phase is only 0.43% of the shared-scale middle span. Offset
  % these two schematic circuit boxes slightly so their labels remain legible;
  % the phase-boundary lines above retain the exact scaled positions.
  \pgfmathsetmacro{\pCDisplay}{\pC-0.50}
  \pgfmathsetmacro{\pDDisplay}{\pD+0.50}

  % Bottom: the two-register quantum circuit abstraction.
  \def\WireLeft{0.24}
  \pgfmathsetmacro{\WireRight}{\PlotRight+0.82}
  \def\XWire{4.42}
  \def\YWire{2.98}
  \draw[wire] (\WireLeft,\XWire) -- (\WireRight,\XWire);
  \draw[wire] (\WireLeft,\YWire) -- (\WireRight,\YWire);

  \node[anchor=east,font=\large,text=ink] at (\WireLeft,\XWire)
    {$\lvert x_p\rangle$};
  \node[anchor=east,font=\large,text=ink] at (\WireLeft,\YWire)
    {$\lvert y_p\rangle$};
  \node[anchor=west,font=\large,text=ink] at (\WireRight,\XWire)
    {$\lvert x_q\rangle$};
  \node[anchor=west,font=\large,text=ink] at (\WireRight,\YWire)
    {$\lvert y_q\rangle$};

  % 1: sequential coordinate subtractions on the two registers.
  \node[gate,minimum width=0.82cm] (subx) at (\pA,\XWire) {$-x_r$};
  \node[gate,minimum width=0.82cm] (suby) at (\pA,\YWire) {$-y_r$};

  % 2: in-place modular inverse/division, coupling the two register paths.
  \node[twowiregate] (inverse) at (\pB,{(\XWire+\YWire)/2})
    {$\mathrm{inv}_p$};

  % 3: classical-coordinate triple add on the x path.
  \node[gate,minimum width=1.12cm] (add3x) at (\pCDisplay,\XWire)
    {$+3x_r$};

  % 4 and 5: the square-subtract and forward multiplication blocks.
  \node[twowiregate] (square) at (\pDDisplay,{(\XWire+\YWire)/2})
    {$\mathrm{sq}^{-}_p$};
  \node[twowiregate] (multiply) at (\pE,{(\XWire+\YWire)/2})
    {$\mathrm{mul}_p$};

  % Filled output markers from the original sketch: lower after inverse,
  % upper after square, and lower after multiplication.
  \coordinate (inverseout) at (inverse.east |- 0,\YWire);
  \coordinate (squareout) at (square.east |- 0,\XWire);
  \coordinate (multiplyout) at (multiply.east |- 0,\YWire);
  \foreach \marker in {inverseout,squareout,multiplyout} {
    \fill[ink]
      ($(\marker)+(0,-0.075)$) --
      ($(\marker)+(0, 0.075)$) --
      ($(\marker)+(0.15,0)$) -- cycle;
  }

  % 6: restore the canonical output coordinates.
  \node[gate,minimum width=0.84cm,font=\scriptsize] (rsub) at (\pF,\XWire)
    {$x_r-\mathord{\cdot}$};
  \node[gate,minimum width=0.82cm] (subyfinal) at (\pF,\YWire)
    {$-y_r$};

  % Dashed grey phase guides: each graph interval fans into the circuit block
  % that implements it, following the hand-drawn mapping in the reference.
  \begin{scope}[on background layer]
    \PhaseGuidePair{\xA}{\xB}{subx}
    \PhaseGuidePair{\xB}{\xC}{inverse}
    \PhaseGuidePair{\xC}{\xD}{add3x}
    \PhaseGuidePair{\xD}{\xE}{square}
    \PhaseGuidePair{\xE}{\xF}{multiply}
    \PhaseGuidePair{\xF}{\PlotRight}{rsub}
  \end{scope}

  % Small bundle marks: each horizontal line abstracts a 256-qubit register.
  \foreach \yy in {\XWire,\YWire} {
    \draw[ink,line width=0.45pt]
      ({\WireLeft+0.17},{\yy-0.18}) -- ({\WireLeft+0.31},{\yy+0.18});
    \node[anchor=south,font=\tiny,text=ink!75] at
      ({\WireLeft+0.24},{\yy+0.22}) {$256$};
  }

\end{tikzpicture}


==> unused/06-methods.tex <==
\section{Methods and Reproducibility Studies}
\label{sec:methods}

%\jieyi{Add experiment results per Craig Gidney's suggestion: Something I would recommend doing is to iterate over all of the existing entries on the leaderboard and compute the error adjusted volume (just sample ten million times instead of 10000 times in order to estimate the error rate). I bet you see the cost curve go the wrong way (a little, not a lot) when people started using gpus to grind for lucky passes.}

\subsection{Benchmark Evaluation and Resource Accounting}
\label{sec:benchmark-evaluation-method}
\francesco{Prepared the evaluator-semantics, validity-tier, held-out-success,
and artifact-integrity methodology.}

\paragraph{Frozen evaluator boundary.}
The trusted evaluator consumes the serialized operation stream emitted by the
untrusted circuit builder. Before simulation it rejects malformed records and
gate operands that violate the operation contract. It then derives a
submission-dependent SHAKE256 stream by hashing the domain tag, operation
count, gate kinds, and every serialized operand. This stream supplies both the
mixed-addition test inputs and the random outcomes used to model reset and
measurement-reset operations. The evaluator revision is part of the experiment
and must therefore be frozen alongside every reported result.

For each test input, the evaluator loads the first affine point into two quantum
registers and the second point into two classical-bit registers, executes the
submitted operation stream once in the forward direction, and compares the two
quantum output coordinates with the classical \texttt{secp256k1} reference
sum. It separately requires zero accumulated phase and zero residual value on
every non-output qubit after the forward execution. The output registers are
cleared before this last scan. Reset and measurement-reset operations also
clear their target qubits and transfer a dirty target into the randomized phase
channel. Consequently, the ancilla counter is a final-state cleanup check,
while dirty-reset behaviour is detected statistically through the phase test;
the evaluator does not perform a deterministic cleanliness assertion at every
deallocation site.

The evaluator does not construct or execute a gate-reversed inverse stream.
Reversibility is supported by the validated reversible operation set together
with forward functional, phase, and cleanup checks, rather than by an
independent forward--reverse identity experiment.

\paragraph{Resource quantities.}
Let $I$ be the set of live validation inputs. For input $i\in I$, let $T_i$ be
the number of executed Toffoli-class operations after classical conditions are
resolved. The benchmark reports
\[
  \bar T=\frac{1}{|I|}\sum_{i\in I}T_i,
  \qquad S=Q\,\operatorname{round}(\bar T),
\]
where $Q$ is one plus the largest qubit identifier referenced by the serialized
stream. Classical control bits and Clifford operations do not contribute to
the score. The detailed results log retains $\bar T$ to three decimal places;
the canonical \texttt{score.json} rounds it before multiplying by $Q$. We use
the rounded leaderboard value for comparisons between published submissions
and retain the unrounded mean when reproducing a run.

At the evidence-cut evaluator revision
\texttt{60d61859fa6965eba53634f91877b1141a6f9dce}, the configured value
$9{,}024$ was an attempted-draw target. Degenerate point pairs were skipped
without replacement, so the printed \texttt{n\_shots}, not the configured
constant alone, is the authoritative denominator for a frozen replay. A later
hardening patch replenishes rejected candidates until exactly $9{,}024$ live
tests are collected; that behaviour is prospective and is not attributed
retroactively to the cutoff results.

\paragraph{Three validity tiers.}
We distinguish claims by the evidence that supports them:
\begin{enumerate}
  \item \emph{Evaluator-clean} means that value, phase, final-state cleanup,
  and structural checks all pass on the deterministic circuit-dependent
  support. It is the admission condition for a scored run, not an all-input
  proof.
  \item \emph{Held-out robust} additionally means that the complete operation
  stream was frozen before testing on an independently committed input domain.
  We report the number of held-out trials, each failure channel, and a binomial
  confidence interval for the success probability $p$.
  \item \emph{Structurally justified} is reserved for transformations supported
  by an algebraic argument, exhaustive bounded-state proof, or equivalent
  all-input invariant whose stated preconditions cover the admitted domain.
\end{enumerate}
These labels describe different evidence levels and are not inferred from a
submission's leaderboard status or note alone.

\paragraph{Held-out success and retry-adjusted score.}
Inputs used to select a nonce, truncation window, schedule, or any other circuit
parameter are optimization data and cannot also estimate $p$. After freezing
the byte-identical operation stream, a held-out study must use a versioned
evaluator variant whose intentional differences are limited to a precommitted,
domain-separated input stream and trial budget. If $k$ of $N$ independent
held-out trials pass all failure channels, we report $\hat p=k/N$ with an exact
binomial interval. In particular, $k=N$ does not establish $p=1$: the
one-sided $(1-\alpha)$ Clopper--Pearson lower bound is
$p_{\mathrm L}=\alpha^{1/N}$, corresponding to an unseen-error upper bound
$1-p_{\mathrm L}\approx-\ln(\alpha)/N$.

The diagnostic quantity
\[
  S_{\mathrm{retry}}=\frac{Q\bar T}{p}
\]
is an expected-retry score for one fixed primitive only when a failure is
detectable, the entire primitive can be restarted, trials are independent, and
their cost distribution is stable. It is not directly the cost of a coherent
Shor computation. If a larger computation contains $L$ independent vulnerable
invocations with common success probability $p$, its no-failure probability is
approximately $p^L$; correlations and input-dependent errors invalidate even
that simplification. We therefore report $Q\bar T/p$ as a robustness diagnostic
and keep attack-level reliability claims separate.

\paragraph{Artifact manifest and reproduction levels.}
For every selected operating point, the artifact manifest records the
submission identifier, circuit-source reference or deposited patch, hash of the
\texttt{src/point\_add} tree, evaluator commit, toolchain and lockfile hashes,
hash of \texttt{ops.bin}, Fiat--Shamir domain, actual \texttt{n\_shots}, and the
resulting \texttt{score.json}. We distinguish numerical reconstruction from the
API, circuit replay under a frozen evaluator, and toolchain-complete rebuild.
Only the latter two execute the circuit, and only the final level also rebuilds
the serialized stream from archived source. This hierarchy prevents a
leaderboard row or source note from being presented as a circuit-level
reproduction when the underlying source artifact is unavailable.




\subsection{Frontier Data and Point-Selection Reconstruction}
\label{sec:frontier-reconstruction-method}

\paragraph{Scope.}
This subsection reconstructs the archive rows and point-selection rules used
for the frontier analysis. It does not rerun the selected circuits through the
evaluator. Circuit-level reproduction would additionally require an evaluator
replay of the corresponding source commits. The analysis below covers the
historical display selection and three cross-sectional $(Q,T)$ admission
rules.

\paragraph{Evidence cut and sources.}
\Cref{tab:external-pa-comparison} reports the Google/Babbush low-gate point at
$Q=1{,}425$ and $T=2{,}100{,}000$. Their product is
$2{,}992{,}500{,}000$; we interpret the 50\% milestone as half this value,
$1{,}496{,}250{,}000$. The first promoted submission at or below this
threshold is \texttt{8e9c9a2}, with $Q=1{,}151$, $T=1{,}299{,}453$, and
$QT=1{,}495{,}670{,}403$. Its promoted source commit is
\texttt{60d61859fa69}. We place the evidence cut at 26 July 2026, 09:21:55
UTC, when that submission's API record was last updated.

Quantitative claims use a frozen response from the official submissions API,
fetched on 27 July. It contains 831 rows, of which 826 were created by the
evidence cut and 576 carry structured $Q$ and $T$ metrics. None of the 826
rows was updated after the cut. The response is retrospective and exposes no
pagination or completeness contract, so these counts describe the pinned
response rather than an asserted complete historical database.

The second source is the 80-row contribution chronology used for Section~5.
Submission identifiers, status fields, metrics, timestamps, and commit
references come from the API. The chronology supplies editorial selections and
mechanism labels. Joining the two sources repairs two spreadsheet-coerced
submission identifiers and two commit references without changing any metric;
all 80 chronology rows reconcile.

\paragraph{Historical display selection.}
The overlay is a manifest-selected editorial set, not a statistical sample or
an automatically discovered set of transitions. It contains 15 points: the
initial baseline, nine product milestones selected in the chronology, the
first 50\%-threshold crossing, and four low-$Q$ foreground rows. Coordinates
come from the API. The chronology supplies labels only for rows it contains.


\paragraph{Pareto construction and admission sensitivity.}
For duplicate $(Q,T)$ coordinates, we retain the earliest submission. After
sorting by increasing $Q$ and then increasing $T$, we keep a point exactly when
its $T$ value is below the running minimum. This implements the dominance rule
in Section~5.

Section~5 admits six rejected low-$Q$
rows on the basis of public validation notes and combines them with promoted
rows. At the evidence cut, that rule produces eight non-dominated points: the
six existing low-$Q$ points and promoted submissions \texttt{8e9c9a2} and
\texttt{a536a48}. The supplementary curation rule is not expressed as a
deterministic predicate over the public fields. We therefore reproduce the
eight-point set as Section~5's editorial selection rather than treating it as
an exhaustive archive-wide frontier.

To measure sensitivity to the admission rule, we compute two alternatives. A
public-note parser requires an explicit 9,024-instance run and zero failures in
each of the classical, phase, and ancilla channels; it produces 16
non-dominated points. A broader calculation includes every pre-cut row carrying
structured API $Q$ and $T$ metrics; it produces 15. The public API does not
document structured metrics as a validation record. We therefore call the
second population \emph{API-metric-bearing}, not \emph{validator-clean}.

\paragraph{Rebuild package.}
The companion package pins the API response and chronology by SHA-256 and
contains the selection manifest, offline reconstruction script, tests, output
tables, and figures. Reproducing these results requires a versioned release of
that package.

\subsection{Ablation Studies}
\label{sec:ablation-studies}
\francesco{Prepared the ablation protocol separating circuit transformations,
support selection, and interaction effects. Numerical results remain pending.}

The public score can change because the emitted circuit changes, because the
submission-dependent validation support changes, or because both change
together. We therefore do not attribute a parent--child score difference to a
named optimization from the commit message alone. An ablation begins by
classifying the diff into (i) semantic circuit-body edits, (ii) identity-tail or
nonce edits that reselect the Fiat--Shamir support, (iii) explicit padding, and
(iv) build or instrumentation changes. Ambiguous or inseparable diffs are
reported as compound interventions.

\paragraph{Crossed circuit and support comparison.}
When the source permits the circuit-body edit and the nonce tail to be varied
independently, we rebuild the four combinations of parent/child body and
parent/child tail. For each combination we record the serialized-operation
hash, peak width, static Toffoli count, executed-Toffoli mean, actual
\texttt{n\_shots}, and the value, phase, and cleanup failure channels. These
four official-evaluator runs expose interaction: the effect of a body change
need not be constant across the two selected supports, so we report the full
$2\times2$ table rather than forcing an additive decomposition.

The same frozen operation streams are then compared on one common,
domain-separated held-out support using the protocol of
\Cref{sec:benchmark-evaluation-method}. A reduction in static gates or in
executed work on common inputs supports a circuit-level explanation. A change
that appears only under the submission-selected support is reported as support
selection. If the body and tail cannot be crossed without changing compilation
or qubit allocation, the intervention fails this ablation and remains bundled.

\paragraph{Mechanism-level ablation.}
For a commit containing several transformations, we construct forward-inclusion
and leave-one-out variants from a common pinned parent whenever the variants
build and validate. The order is preregistered because reversible optimizations
can interact through ancilla lifetimes, classical conditions, and compiler
simplification. We report every attempted variant, including build failures and
validator failures; successful variants alone cannot estimate the marginal
value of a mechanism. Width and executed work are reported separately before
their product, and no marginal contribution is claimed when the mechanism
cannot be isolated from its enabling changes.


\subsection{Trajectory Reproducibility Studies}
\label{sec:trajectory-reproducibility-studies}
\francesco{Prepared the trajectory-reproduction protocol and explicit failure
criteria. Numerical reconstruction, circuit replay, and rebuild are kept distinct.}

The trajectory is reproduced at three levels. A \emph{ledger reconstruction}
recreates dated tables and figures from a pinned API response and chronology.
A \emph{circuit replay} executes a deposited serialized operation stream under
the frozen evaluator. A \emph{toolchain-complete rebuild} additionally rebuilds
that stream from the archived source and lockfiles. Passing a weaker level is
not evidence that a stronger level passed.

For each displayed operating point, the reproduction matrix records the
submission identifier, source or patch reference, source-tree hash, evaluator
commit, operation-stream hash, actual validation count, reproduced $(Q,T)$,
and outcome at each level. A replay passes only if all failure channels are zero
and the reproduced width and rounded score match the deposited record; we also
retain the unrounded executed-Toffoli mean. A rebuild passes only if the
operation-stream hash matches. Toolchain drift, an unavailable source artifact,
or a differing stream is a reported failure rather than a value silently copied
from the public API.

\paragraph{Chronology and negative evidence.}
The study pins one evidence cut per analysis and rejects rows updated beyond
that cut. Duplicate coordinates retain the earliest admissible row under the
stated rule. We preserve missing sources, rejected runs, and unavailable
intermediate commits in the matrix because they bound what can be claimed about
the optimization path. The resulting chronology describes reproducible public
artifacts; it does not reconstruct unlogged local attempts or prove that the
displayed sequence was the only path to the final circuit.


\subsection{Experiments for the Proposed Consolidated Autoresearch Framework} \label{sec:experiments-for-consolidated-autoresearch-framework}

